Hyperspectral Neural Radiance Fields

Hyperspectral Imagery (HSI) has been used in many applications to non-destructively determine the material and/or chemical compositions of samples. There is growing interest in creating 3D hyperspectral reconstructions, which could provide both spatial and spectral information while also mitigating common HSI challenges such as non-Lambertian surfaces and translucent objects. However, traditional 3D reconstruction with HSI is difficult due to technological limitations of hyperspectral cameras. In recent years, Neural Radiance Fields (NeRFs) have seen widespread success in creating high quality volumetric 3D representations of scenes captured by a variety of camera models. Leveraging recent advances in NeRFs, we propose computing a hyperspectral 3D reconstruction in which every point in space and view direction is characterized by wavelength-dependent radiance and transmittance spectra. To evaluate our approach, a dataset containing nearly 2000 hyperspectral images across 8 scenes and 2 cameras was collected. We perform comparisons against traditional RGB NeRF baselines and apply ablation testing with alternative spectra representations. Finally, we demonstrate the potential of hyperspectral NeRFs for hyperspectral super-resolution and imaging sensor simulation. We show that our hyperspectral NeRF approach enables creating fast, accurate volumetric 3D hyperspectral scenes and enables several new applications and areas for future study.

==> 3b-approach-hypernerf-OLD.tex <==
% \patrick{IMO CV people like naming their approaches. In the title you picked HS-NeRF, which is cool. You might plug that in here as many times as possible, so this section header is HS-NeRF, and many of the refs in the text can be replaced with HS-NeRF}
We build our implementation of HS-NeRF upon nerfstudio's ``nerfacto'' implementation \cite{nerfstudio}.

As compared to a $(H, W, 3)$ RGB image, a hyperspectral image can be represented by a $(H, W, N)$ tensor, where $H$ and $W$ are the height and width of the image, and $N$ is the number of channels/wavelengths.

In our final implementation, we represent both color emission and color absorption as continuous spectra -- intensities as functions of wavelength -- by predicting latent vectors representing parameters of learned spectral plots which are evaluated for a given wavelength with decoders.
% In our final implementation, we represent both color emission and color absorption as continuous spectra -- intensities as functions of wavelength -- by predicting latent vectors $\bm{\Theta}_c, \bm{\Theta}_\sigma$ representing parameterizations of learned spectral plots which are evaluated with decoders $d_c(\lambda~;~\bm{\Theta}_c) = c^\lambda$ and $d_\sigma(\lambda~;~\bm{\Theta}_\sigma) = \sigma^\lambda$.

In this section, we describe the implementation details, as well as several alternative architectures tested in our ablations, for predicting color emission and absorption spectra, as well as a ray sample proposal network that predicts a wavelength-dependent proposal density.
% We introduce 3 primary changes to the nerfacto architecture: (1) the color emission network is changed to output a color spectrum, (2) the color absorption network is changed to output a wavelength-dependent absorption spectrum, and (3) the proposal network is changed to output a wavelength-dependent proposal spectrum.

\subsection{Color Emittance Spectrum Prediction}
Whereas the original and nerfacto networks predict a 3-channel color vector, we choose to predict a continuous color emission spectrum.  We also discuss several alternative approaches and compare their performance in the ablations section (\ref{ssec:ablations}).

Specifically, in this work, we study (1) predicting the color \emph{discretely} as an N-dimensional vector, or (2) predicting the \emph{continuous} intensity vs wavelength spectral plot.
% Whereas the original and nerfacto networks predict a 3-channel color vector, we can predict the 128 channels/wavelengths imaged by the hyperspectral camera in several ways.
% Defining $N=128$ as the number of channels we wish the NeRF to predict, we may choose to either (1) predict the color \emph{discretely} as an N-dimensional vector, or (2) predict the \emph{continuous} intensity vs wavelength spectral plot.
Furthermore in (2), we may either (2a) treat wavelength as an additional ``spatial'' input dimension or (2b) predict a latent vector that represents the spectral plot and use a decoder to evaluate the spectrum at a given wavelength.  We find in the ablations section (\ref{ssec:ablations}) that (2b) is the most effective.

More formally, the original and nerfacto networks output the color intensity at a point on a ray as
\begin{align}
  % F_0 &: \bm{c}(\bm{x}, \bm{d}) = (r, g, b)
  E_0 &: (\bm{x}, \bm{d}) \rightarrow \bm{c} := (r, g, b)
\end{align}
where $\bm{x} := (x, y, z)$ is the location of the point and $\bm{d} := (\theta, \phi)$ describes the view direction of the ray.  We propose the following 3 architectures for predicting emitted (hyperspectral) color:
\begin{align}
  E_1 &: (\bm{x}, \bm{d}) \rightarrow (c^{\lambda_1}, \ldots, c^{\lambda_N}) \\ % & &: \mathbb{R}^5 \rightarrow \mathbb{R}^N \\
  E_{2a} &: (\bm{x}, \bm{d}, \lambda) \rightarrow c^\lambda \\ % & &: \mathbb{R}^6 \rightarrow \mathbb{R} \\
  E_{2b} &: (\lambda~;~\bm{\Theta}_c(\bm{x}, \bm{d})) \rightarrow c^\lambda    % & &: \mathbb{R}^{1+n_\Theta} \rightarrow \mathbb{R}
\end{align}
where
  $c^\lambda$ denotes the scalar emitted (color) intensity at wavelength $\lambda$,
  $\lambda$ denotes the query wavelength,
  $\bm{\Theta}_c(\bm{x}, \bm{d}): \mathbb{R}^5 \rightarrow \mathbb{R}^{n_\Theta}$ is a neural network that maps the ray's location and view direction to a latent vector $\bm{\Theta}$, and
  $n_\Theta$ is the dimensionality of the latent vector.

Implementation details are provided in \ref{ssec:implementation}.

\subsection{Color Transmittance Spectrum Prediction}
Similarly, the color transmittance spectrum describes a wavelength-dependent volume density.
In other words, instead of using a scalar density field to describe the transparency of the scene, we investigate the possibility of using a wavelength-dependent density field.

Although wavelength-dependent transmittance can also be applied to RGB scenes, it is particularly interesting for hyperspectral imagery due to the fact that many materials are transparent in visible wavelengths but opaque in IR or vice-versa.

In the original and nerfacto NeRF implementations, the volume density is given by a scalar function $\sigma(\bm{x})$ of location $\bm{x} = (x, y, z)$.
Instead, we may choose to model the volume density to be wavelength-dependent in much the same way as we treated color emission: $F_1$ outputs 128 density channels instead of 1, $F_{2a}$ appends wavelength to the \emph{position} vector before the positional encoding, and $F_{2b}$ outputs a latent vector $\bm{\Theta}_\sigma$ instead of the scalar density that is then decoded the same way as in the color emission.

\subsection{Wavelength-dependent Proposal Network}
When choosing to use a wavelength-dependent volume density, it is also natural to make the sample proposal network (analagous to the ``coarse'' network in the original NeRF paper) wavelength-dependent.  We can again use the same 3 architectures as in the color emission section.

% \subsection{Dummy}

% The original NeRF looks like:
% $$ f(x, y, z, \theta, \phi) = (R, G, B, \sigma) $$.

% We propose 3 different ways to extend this to hyperspectral NeRF:
% \begin{enumerate}
%   \item $ f(x, y, z, \theta, \phi) = (c_0, \ldots, c_{127}, \sigma) $
%   \item $ f(x, y, z, \theta, \phi) = (c_0, \ldots, c_{127}, \sigma_0, \ldots, \sigma_{127}) $
%   \item $ f(x, y, z, \theta, \phi, \lambda) = (c_\lambda, \sigma_\lambda) $.
% \end{enumerate}

% Furthermore, we may choose to implement these neural network functions in different architectures.

% We start from nerfstudio's ``nerfacto'' implementation (cite).  We don't modify the proposal network (aka coarse network) at all. blah blah details

\subsection{Implementation} \label{ssec:implementation}
We find that using $F_{2b}$ for both the emission and absorption networks and the default nerfacto proposal network (i.e. $F_0$) works best for our experiments, though we also test several other combinations in \ref{ssec:ablations}.

Thus, in our final implementation, we represent both color emission and color absorption as continuous spectra -- intensities as functions of wavelength -- by predicting latent vectors $\bm{\Theta}_c, \bm{\Theta}_\sigma$ representing parameterizations of learned spectral plots which are evaluated with decoders $d_c(\lambda~;~\bm{\Theta}_c) = c^\lambda$ and $d_\sigma(\lambda~;~\bm{\Theta}_\sigma) = \sigma^\lambda$.
\todo{fix notation, and maybe cut this paragraph.}




\todo{move this to implementation section} Implementation-wise, $E_1$ uses the same network as in the nerfacto model except the last layer of the color prediction MLP outputs 128 channels instead of 3.  $E_{2a}$ uses the same network as in the nerfacto model except the wavelength is appended to the direction vector before the spherical encoding.  Finally, $E_{2b}$ uses the same network as in the the nerfacto model except the color prediction network outputs an $n_\Theta$-dimensional latent vector $\bm{\Theta}$ instead of a 3-channel color vector.  The latent vector is then appended to a 4-frequency sinusoidal encoded wavelength and decoded by a 2-layer MLP that outputs the color intensity at a given wavelength.


==> tables/ablation_auto.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 13.242 &  0.818 &  0.160     &      16.493 &  0.819 &  0.317     &      15.335 &  0.588 &  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      & 12.572 &  0.805 &  0.194     &      16.358 &  0.809 &  0.332     &      14.375 &  0.431 &  0.709 \\
\bm{C}_2 & \sigma_2 & P_0      & 12.149 &  0.797 &  0.209     &      16.219 &  0.777 &  0.303     &      15.708 &  0.642 &  0.568 \\
(ours)~\bm{C} & \sigma & P_0   & 11.622 &  0.775 &  0.202     &      16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733 \\
\bm{C} & \sigma & P_\lambda    & 11.602 &  0.762 &  0.213     &      14.637 &  0.710 &  0.283     &      13.221 &  0.399 &  0.663 \\


==> tables/ablation_auto_alt.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 18.703 &  0.883 &  0.096     &      15.820 &  0.756 &  0.234     &      15.335 &  0.588 &  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      & 18.432 &  0.873 &  0.106     &      15.882 &  0.760 &  0.247     &      14.375 &  0.431 &  0.709 \\
(ours)~\bm{C}_{\phantom{~}} & \sigma_0 & P_0  & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489 \\
\bm{C}_{\phantom{~}} & \sigma & P_0   & 17.477 &  0.863 &  0.090     &      16.532 &  0.792 &  0.237     &       7.958 &  0.333 &  0.621 \\
\bm{C}_2 & \sigma_2 & P_0      & 19.744 &  0.895 &  0.076     &      16.393 &  0.776 &  0.207     &      15.708 &  0.642 &  0.568 \\
\bm{C}_{\phantom{~}} & \sigma & P_\lambda    & 17.494 &  0.851 &  0.128     &      15.265 &  0.704 &  0.312     &      13.221 &  0.399 &  0.663 \\


==> tables/ablation_auto_bayspec.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 20.279 &  0.734 &  0.295     &      19.084 &  0.705 &  0.530     &      20.102 &  0.729 &  0.399 \\
\bm{C}_1 & \sigma_1 & P_0      & 20.128 &  0.729 &  0.305     &      19.933 &  0.678 &  0.495     &      19.857 &  0.726 &  0.372 \\
(ours)~\bm{C}_{\phantom{~}} & \sigma_0 & P_0  & 20.315 &  0.726 &  0.297     &      19.428 &  0.687 &  0.523     &      20.162 &  0.740 &  0.409 \\
\bm{C}_{\phantom{~}} & \sigma & P_0   & 20.095 &  0.705 &  0.320     &      18.942 &  0.653 &  0.514     &      19.596 &  0.729 &  0.409 \\
\bm{C}_2 & \sigma_2 & P_0      & 21.259 &  0.711 &  0.319     &      18.989 &  0.595 &  0.568     &      19.732 &  0.561 &  0.434 \\
\bm{C}_{\phantom{~}} & \sigma & P_\lambda    & 15.031 &  0.667 &  0.351     &      15.930 &  0.626 &  0.556     &      15.700 &  0.485 &  0.484 \\


==> tables/ablation_auto_colorized.tex <==
\bm{C}_1 & \sigma_0 & P_0      &\cellcolor[rgb]{0.5,1,0.5} 13.242 &\cellcolor[rgb]{0.5,1,0.5}  0.818 &\cellcolor[rgb]{0.5,1,0.5}  0.160     &\cellcolor[rgb]{0.5,1,0.5}      16.493 &\cellcolor[rgb]{0.5,1,0.5}  0.819 &\cellcolor[rgb]{0.9999963865521223,1,0.9999963865521223}  0.317     &\cellcolor[rgb]{0.6805095915200885,1,0.6805095915200885}      15.335 &\cellcolor[rgb]{0.9257498479433259,1,0.9257498479433259}  0.588 &\cellcolor[rgb]{0.5,1,0.5}  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      &\cellcolor[rgb]{0.9973803162478166,1,0.9973803162478166} 12.572 &\cellcolor[rgb]{0.9643734071913941,1,0.9643734071913941}  0.805 &\cellcolor[rgb]{0.9999824713964786,1,0.9999824713964786}  0.194     &\cellcolor[rgb]{0.7650372650060329,1,0.7650372650060329}      16.358 &\cellcolor[rgb]{0.8089896189767647,1,0.8089896189767647}  0.809 &\cellcolor[rgb]{1.0,1,1.0}  0.332     &\cellcolor[rgb]{0.9088677398998146,1,0.9088677398998146}      14.375 &\cellcolor[rgb]{0.9999940930116535,1,0.9999940930116535}  0.431 &\cellcolor[rgb]{0.9999999991121137,1,0.9999999991121137}  0.709 \\
\bm{C}_2 & \sigma_2 & P_0      &\cellcolor[rgb]{0.9999914806828285,1,0.9999914806828285} 12.149 &\cellcolor[rgb]{0.9954525264911352,1,0.9954525264911352}  0.797 &\cellcolor[rgb]{0.9999999999970022,1,0.9999999999970022}  0.209     &\cellcolor[rgb]{0.8987826233403338,1,0.8987826233403338}      16.219 &\cellcolor[rgb]{0.9961500680606966,1,0.9961500680606966}  0.777 &\cellcolor[rgb]{0.9973637342763831,1,0.9973637342763831}  0.303     &\cellcolor[rgb]{0.5,1,0.5}      15.708 &\cellcolor[rgb]{0.5,1,0.5}  0.642 &\cellcolor[rgb]{0.7905480560577024,1,0.7905480560577024}  0.568 \\
(ours)~\bm{C} & \sigma & P_0   &\cellcolor[rgb]{1.0,1,1.0} 11.622 &\cellcolor[rgb]{0.9999997727398665,1,0.9999997727398665}  0.775 &\cellcolor[rgb]{0.9999999258453892,1,0.9999999258453892}  0.202     &\cellcolor[rgb]{0.5,1,0.5}      16.493 &\cellcolor[rgb]{0.9411790890013152,1,0.9411790890013152}  0.798 &\cellcolor[rgb]{0.8295739537151602,1,0.8295739537151602}  0.288     &\cellcolor[rgb]{1.0,1,1.0}       7.192 &\cellcolor[rgb]{1.0,1,1.0}  0.331 &\cellcolor[rgb]{1.0,1,1.0}  0.733 \\
\bm{C} & \sigma & P_\lambda    &\cellcolor[rgb]{1.0,1,1.0} 11.602 &\cellcolor[rgb]{1.0,1,1.0}  0.762 &\cellcolor[rgb]{1.0,1,1.0}  0.213     &\cellcolor[rgb]{1.0,1,1.0}      14.637 &\cellcolor[rgb]{1.0,1,1.0}  0.710 &\cellcolor[rgb]{0.5,1,0.5}  0.283     &\cellcolor[rgb]{0.9841851049096417,1,0.9841851049096417}      13.221 &\cellcolor[rgb]{0.9999998751308253,1,0.9999998751308253}  0.399 &\cellcolor[rgb]{0.9999604428172743,1,0.9999604428172743}  0.663 \\


==> tables/old/ablation.tex <==
$$
\begin{array}{ccc | ccc ccc}
  % \rotatebox{-90}{Emittance Network} & \rotatebox{-90}{Transmittance Network} & \rotatebox{-90}{Proposal Network} & \multicolumn{3}{c}{Basil} & \multicolumn{3}{c}{Tools} \\
  \multicolumn{3}{c|}{\text{Network}} & \multicolumn{3}{c}{\text{Basil}} & \multicolumn{3}{c}{\text{Tools}} \\
  \multicolumn{3}{c|}{\text{Archictecure}} & \text{\PSNR} & \text{\SSIM} & \text{\LPIPS} & \text{\PSNR} & \text{\SSIM} & \text{\LPIPS} \\
   \cmidrule(lr){1-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
  %  \text{\hspace*{-6.5em}(HS-NeRF)\hspace*{0.5em}} 
  \input{tables/ablation_auto}
\end{array}
$$

==> tables/old/ablation_auto.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 16.493 &  0.819 &  0.317     &      15.335 &  0.588 &  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      & 16.358 &  0.809 &  0.332     &      14.375 &  0.431 &  0.709 \\
\bm{C}_2 & \sigma_2 & P_0      & 16.219 &  0.777 &  0.303     &      15.708 &  0.642 &  0.568 \\
(ours)~\bm{C} & \sigma & P_0   & 16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733 \\
\bm{C} & \sigma & P_\lambda    & 14.637 &  0.710 &  0.283     &      13.221 &  0.399 &  0.663 \\


==> tables/old/rgb.tex <==
\begin{tabular}[htp]{l ccc ccc ccc ccc} \toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Rosemary} & \multicolumn{3}{c}{Basil} & \multicolumn{3}{c}{Tools} & \multicolumn{3}{c}{Origami} \\
           & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM & \LPIPS & \PSNR & \SSIM & \LPIPS \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
  \input{tables/rgb_auto}
  \bottomrule
\end{tabular}

==> tables/old/rgb_auto.tex <==
nerfacto   & 20.675 &  0.892 &  0.103     &      17.244 &  0.790 &  0.226     &      11.760 &  0.338 &  0.492     &      12.400 &  0.361 &  0.768 \\
Ours-Cont  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &      12.168 &  0.385 &  0.533     &      10.741 &  0.289 &  0.562 \\
Ours-RGB   & 18.601 &  0.865 &  0.083     &      16.780 &  0.765 &  0.212     &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\
Ours-Hyper & 17.702 &  0.870 &  0.094     &      16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733     &      10.359 &  0.453 &  0.693 \\


==> tables/old/rgbauto.tex <==
nerfacto   & 20.675 &  0.892 &  0.103     &      17.244 &  0.790 &  0.226     &      11.760 &  0.338 &  0.492     &      12.400 &  0.361 &  0.768 \\
Ours-Cont  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &        --   &   --   &   --       &      10.741 &  0.289 &  0.562 \\
Ours-RGB   &   --   &   --   &   --       &        --   &   --   &   --       &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\


==> tables/old/wavelength.tex <==
\begin{tabular}[pos]{c ccc ccc cc cc} \toprule
  \# of Wavelengths & \multicolumn{3}{c}{Train Set} & \multicolumn{3}{c}{Unseen Images} & \multicolumn{2}{c}{Unseen Wavelengths} & \multicolumn{2}{c}{Both Unseen} \\
  in Train Set      & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM  & \PSNR & \SSIM  \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
   \input{tables/wavelength_auto}
  \bottomrule
\end{tabular}


==> tables/old/wavelength_auto.tex <==
128        & 20.378 &  0.848 &  0.255 & 16.493 &  0.798 &  0.288 & N/A & N/A & N/A & N/A \\
64         & 19.893 &  0.839 &  0.246 & 16.534 &  0.786 &  0.277 & 20.005 &  0.834 & 16.651 &  0.782 \\
32         & 19.460 &  0.825 &  0.264 & 16.229 &  0.781 &  0.296 & 19.447 &  0.820 & 16.258 &  0.777 \\
16         & 14.592 &  0.759 &  0.272 & 13.586 &  0.717 &  0.306 & 14.656 &  0.759 & 13.641 &  0.717 \\


==> tables/rgb_auto.tex <==
nerfacto   & 18.789 &  0.868 &  0.089     &      16.147 &  0.714 &  0.229     &      11.760 &  0.338 &  0.492     &      10.371 &  0.220 &  0.560 \\
Ours-Cont  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &      12.168 &  0.385 &  0.533     &      10.741 &  0.289 &  0.562 \\
Ours-RGB   & 18.601 &  0.865 &  0.083     &      16.780 &  0.765 &  0.212     &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\
Ours-HS & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489     &      10.359 &  0.453 &  0.693 \\


==> tables/rgb_auto_bayspec.tex <==
nerfacto   & 14.413 &  0.626 &  0.432     &      14.190 &  0.555 &  0.503     &      14.120 &  0.323 &  0.464 \\
Ours-Cont  & 14.171 &  0.626 &  0.437     &      14.306 &  0.543 &  0.507     &      13.868 &  0.382 &  0.414 \\
Ours-RGB   & 14.321 &  0.619 &  0.435     &      14.249 &  0.569 &  0.501     &      15.412 &  0.615 &  0.442 \\
Ours-HS & 20.315 &  0.726 &  0.297     &      19.084 &  0.705 &  0.530     &      20.066 &  0.580 &  0.885 \\


==> tables/wavelength_auto.tex <==
128        & 20.378 &  0.848 &  0.255 & 16.493 &  0.798 &  0.288 & N/A & N/A & N/A & N/A \\
64         & 19.893 &  0.839 &  0.246 & 16.534 &  0.786 &  0.277 & 20.005 &  0.834 & 16.651 &  0.782 \\
32         & 19.460 &  0.825 &  0.264 & 16.229 &  0.781 &  0.296 & 19.447 &  0.820 & 16.258 &  0.777 \\
16         & 14.592 &  0.759 &  0.272 & 13.586 &  0.717 &  0.306 & 14.656 &  0.759 & 13.641 &  0.717 \\


==> tables/wavelength_auto_bayspec.tex <==
128        & 20.550 &  0.730 &  0.294 & 20.315 &  0.726 &  0.297 & N/A & N/A & N/A & N/A \\
64         & 20.947 &  0.735 &  0.461 & 20.701 &  0.732 &  0.459 & 20.979 &  0.736 & 20.732 &  0.733 \\
32         & 20.760 &  0.734 &  0.469 & 20.512 &  0.731 &  0.468 & 20.773 &  0.734 & 20.527 &  0.732 \\
16         & 19.868 &  0.727 &  0.477 & 19.705 &  0.725 &  0.474 & 19.854 &  0.728 & 19.690 &  0.726 \\

